Accelerating Numerical Relativity with Code Generation: CUDA-enabled Hyperbolic Relaxation

Next-generation gravitational wave detectors such as Cosmic Explorer, the Einstein Telescope, and LISA, demand highly accurate and extensive gravitational wave (GW) catalogs to faithfully extract physical parameters from observed signals. However, numerical relativity (NR) faces significant challenges in generating these catalogs at the required scale and accuracy on modern computers, as NR codes do not fully exploit modern GPU capabilities. In response, we extend NRPy, a Python-based NR code-generation framework, to develop NRPyEllipticGPU -- a CUDA-optimized elliptic solver tailored for the binary black hole (BBH) initial data problem. NRPyEllipticGPU is the first GPU-enabled elliptic solver in the NR community, supporting a variety of coordinate systems and demonstrating substantial performance improvements on both consumer-grade and HPC-grade GPUs. We show that, when compared to a high-end CPU, NRPyEllipticGPU achieves on a high-end GPU up to a sixteenfold speedup in single precision while increasing double-precision performance by a factor of 2--4. This performance boost leverages the GPU's superior parallelism and memory bandwidth to achieve a compute-bound application and enhancing the overall simulation efficiency. As NRPyEllipticGPU shares the core infrastructure common to NR codes, this work serves as a practical guide for developing full, CUDA-optimized NR codes.

==> Makefile <==
# Simplified Makefile to compile nrpyelliptic_gpu paper

USE_BIBTEX=yes

# Main target
all: nrpyelliptic_gpu.pdf

# Rule to generate PDF
nrpyelliptic_gpu.pdf: nrpyelliptic_gpu.tex nrpyelliptic_gpu.bbl Makefile \
    roofline_falcon.pdf \
    roofline.pdf \
    instruction_comparison.pdf \
    weak_scaling-falcon.pdf \
    weak_scaling-combined.pdf \
    CPO-combined.pdf \
    cmp.pdf \
    multigrid_comparison.pdf
	pdflatex nrpyelliptic_gpu.tex
ifeq ($(USE_BIBTEX),yes)
	bibtex nrpyelliptic_gpu
	pdflatex nrpyelliptic_gpu.tex
endif
	pdflatex nrpyelliptic_gpu.tex

# Clean up auxiliary files
.PHONY: clean veryclean

clean:
	rm -f nrpyelliptic_gpu.aux nrpyelliptic_gpu.blg nrpyelliptic_gpu.log \
	      nrpyelliptic_gpu.out nrpyelliptic_gpu.toc *~

veryclean: clean
	rm -f nrpyelliptic_gpu.pdf

